On Formalizing Fairness in Prediction with Machine Learning

Machine learning algorithms for prediction are increasingly being used in critical decisions affecting human lives. Various fairness formalizations, with no firm consensus yet, are employed to prevent such algorithms from systematically discriminating against people based on certain attributes protected by law. The aim of this article is to survey how fairness is formalized in the machine learning literature for the task of prediction and present these formalizations with their corresponding notions of distributive justice from the social sciences literature. We provide theoretical as well as empirical critiques of these notions from the social sciences literature and explain how these critiques limit the suitability of the corresponding fairness formalizations to certain domains. We also suggest two notions of distributive justice which address some of these critiques and discuss avenues for prospective fairness formalizations.

==> todo.tex <==
Incorporating new perspectives and material:

Tutorial at FATconference:
https://fatconference.org/static/tutorials/narayanan-21defs18.pdf
Videorecording are here: https://www.youtube.com/channel/UCs16j6ot-CYq-ZqYpO-vqMg/videos
but tutorial is not there.
By I have my notes.

Tutorial at NIPS
http://mrtz.org/nips17/#/

Input received at FRA (check notes)

Fairness in RecSys:
http://proceedings.mlr.press/v81/kamishima18a/kamishima18a.pdf
http://proceedings.mlr.press/v81/burke18a/burke18a.pdf

Cost-sensitive view on fairness measures:
http://proceedings.mlr.press/v81/menon18a/menon18a.pdf

Types of Discrimination Recognized by Courts?:
https://fatconference.org/static/tutorials/schmidt_banking18.pdf

Auditing black box models:
https://arxiv.org/abs/1602.07043
apeared in KAIS

Nabi, R. and Shpitser, I. Fair inference on outcomes. In
Thirty-Second AAAI Conference on Artificial Intelligence,
2018.
https://arxiv.org/abs/1802.08139


http://auditingalgorithms.science/?p=372
